Adversarial score matching and improved sampling for image generation

Denoising Score Matching with Annealed Langevin Sampling (DSM-ALS) has recently found success in generative modeling. The approach works by first training a neural network to estimate the score of a distribution, and then using Langevin dynamics to sample from the data distribution assumed by the score network. Despite the convincing visual quality of samples, this method appears to perform worse than Generative Adversarial Networks (GANs) under the Fr\'echet Inception Distance, a standard metric for generative models. We show that this apparent gap vanishes when denoising the final Langevin samples using the score network. In addition, we propose two improvements to DSM-ALS: 1) Consistent Annealed Sampling as a more stable alternative to Annealed Langevin Sampling, and 2) a hybrid training formulation, composed of both Denoising Score Matching and adversarial objectives. By combining these two techniques and exploring different network architectures, we elevate score matching methods and obtain results competitive with state-of-the-art image generation on CIFAR-10.

==> sections/arxiv_intro.tex <==
\citet{song2019generative} recently proposed a novel method of generating samples from a target distribution through a combination of Denoising Score Matching (DSM) \citep{hyvarinen2005estimation, vincent2011connection, raphan2011least} and Annealed Langevin Sampling (ALS) \citep{welling2011bayesian,roberts1996exponential}. 
Since convergence to the distribution is guaranteed by the ALS, their approach (DSM-ALS) produces high-quality samples and guarantees high diversity. Though, this comes at the cost of requiring an iterative process during sampling, contrary to other generative methods.
%The main benefits of their approach (DSM-ALS) are that it produces relatively high-quality samples and guarantees high diversity due to ALS. The main drawback of DSM-ALS is that generating samples requires many iterations rather than being done in one-shot.

\citet{song2020improved} further improved their approach by increasing the stability of score matching training and proposing theoretically sound choices of hyperparameters. They also scaled their approach to higher-resolution images and showed that DSM-ALS is competitive with other generative models.
\citet{song2020improved} observed that the images produced by their improved model were more visually appealing than the ones from their original work;
however, the reported Fréchet Inception Distance (FID) \citep{heusel2017gans} did not correlate with this improvement. 

Although DSM-ALS is gaining traction, Generative adversarial networks (GANs) \citep{GAN} remain the leading approach to generative modeling. GANs are a very popular class of generative models; they have been successfully applied to image generation \citep{brock2018large,karras2017progressive,karras2019style,karras2020analyzing} and have subsequently spawned a wealth of variants \citep{radford2015unsupervised,miyato2018spectral,jolicoeur2018relativistic,zhang2019self}. The idea behind this method is to train a Discriminator ($D$) to correctly distinguish real samples from fake samples generated by a second agent, known as the Generator ($G$). GANs excel at generating high-quality samples as the discriminator captures features that make an image plausible, while the generator learns to emulate them.

Still, GANs often have trouble generating data from all possible modes, which impedes the diversity of the generated samples. A wide variety of tricks has been developed to address this issue in GANs \citep{kodali2017convergence,WGAN-GP,WGAN,miyato2018spectral,jolicoeur2019connections}. DSM-ALS, on the other hand, does not suffer from such issue since ALS allows for sampling from the full distribution captured by the score network. Nevertheless, the perceptual quality of DSM-ALS higher-resolution images remains so far inferior to those generated by GANs. Generative modeling has also seen some incredible work from \citet{ho2020denoising}, who achieved exceptionally low FID on image generation tasks. Their approach showcased a new diffusion-based method \citep{sohl2015deep, goyal2017variational} that shares close ties with Denoising Score Matching, and used a network architecture derived from that of \citet{salimans2017pixelcnn++}.

In this paper, after introducing the necessary technical background in Section~\ref{sec:back}, we build upon the work and limitations described above to improve DSM-ALS and bring it closer to GANs and the diffusion-based approach from \cite{ho2020denoising}. Our contributions are the following.

In Section \ref{sec:consistent}, we show that the scaling of the additive noise in the ALS proposed by \citet{song2019generative, song2020improved} does not ensure that the levels of noise in the samples will decrease geometrically at inference time, and we hypothesize this incongruity is harmful to the quality of samples. We show how to scale the noise for \em consistent sampling \em by introducing Consistent Annealed Sampling (CAS). CAS is such that the noise level at any time step follows the desired schedule \em as best as possible \em.

In Section \ref{sec:sampling_improvements}, we study the \em expected denoised sample \em (EDS) \citep{robbins1955empirical, miyasawa1961empirical, raphan2011least}. We show that taking the EDS of the last Langevin sample corrects the mismatch observed by~\cite{song2020improved} between the visual quality of generated images in DSM-ALS and their rather high FID. We also provide some intuition behind the phenomenon.

In Section \ref{sec:adversarial}, we further exploit the EDS by presenting a hybrid between GANs and Denoising Score Matching. Our algorithm augments standard DSM with a discriminator that encourages the EDS of the score network to be as realistic as possible. 

In Section \ref{sec:experiments}, we demonstrate that this hybrid method improves the quality of samples without sacrificing their diversity. We also show that the network architecture used used by~\cite{ho2020denoising} significantly improves quality over the RefineNet \citep{lin2017refinenet} architecture used by \citet{song2020improved}. Finally, we study how our two training improvements (hybrid objective, and \citet{ho2020denoising} score network architecture) and sampling improvements (consistent sampling, expected denoised sample) interact by performing an ablation study on the CIFAR-10 and LSUN-Churches generation tasks. The code to replicate our experiments is publicly available at 
https://www.dropbox.com/sh/hulwb6985gkx1fo/AAA5ct6P1z0mu\_JEt5ySaC0Ea?dl=0
%https://github.com/AlexiaJM/AdversarialConsistentScoreMatching.

==> sections/authors.tex <==

 \author{Alexia Jolicoeur-Martineau\thanks{First two authors have equal contributions} \\
 Department of Computer Science\\
 University of Montreal
 \And 
 Rémi Piché-Taillefer\textsuperscript{*} \\
 Department of Computer Science\\
 University of Montreal
 \And
 Rémi Tachet des Combes \\
 Microsoft Research Lab \\
 Microsoft Research Montreal
 \And
 Ioannis Mitliagkas \\
 Department of Computer Science\\
 University of Montreal
}
